Hybrid Temporal Computing for Lower Power Hardware Accelerators

In this paper, we propose a new hybrid temporal computing (HTC) framework that leverages both pulse rate and temporal data encoding to design ultra-low energy hardware accelerators. Our approach is inspired by the recently proposed temporal computing, or race logic, which encodes data values as single delays, leading to significantly lower energy consumption due to minimized signal switching. However, race logic is limited in its applications due to inherent restrictions. The new HTC framework overcomes these limitations by encoding signals in both temporal and pulse rate formats for multiplication and in temporal format for propagation. This approach maintains reduced switch energy while being general enough to implement a wide range of arithmetic operations. We demonstrate how HTC multiplication is performed for both unipolar and bipolar data encoding and present the basic designs for multipliers, adders, and MAC units. Additionally, we implement two hardware accelerators: a Finite Impulse Response (FIR) filter and a Discrete Cosine Transform (DCT)/iDCT engine for image compression and DSP applications. Experimental results show that the HTC MAC has a significantly smaller power and area footprint compared to the Unary MAC design and is orders of magnitude faster. Compared to the CBSC MAC, the HTC MAC reduces power consumption by $45.2\%$ and area footprint by $50.13\%$. For the FIR design, the HTC design significantly outperforms the Unary design on all metrics. Compared to the CBSC design, the HTC-based FIR filter reduces power consumption by $36.61\%$ and area cost by $45.85\%$. The HTC-based DCT filter retains the quality of the original image with a decent PSNR, while consuming $23.34\%$ less power and occupying $18.20\%$ less area than the CBSC MAC-based DCT filter.

==> old_sc_review_by_sachin.tex <==
\section{Review of related works}

\subsection{Stochastic Computing}
Stochastic computing (SC) is recognized as a novel computational framework that offers economical and robust solutions for executing complex arithmetic operations, such as multiplication. Unlike traditional binary systems where data is represented positionally, SC employs non-positional bit-streams uniformly distributed. Within this framework, numerical values are encoded through the probability of a bit being '1' instead of '0'. Operations are conducted on these stochastic bit streams, which may either be deterministic, consisting uniformly of all '1s' followed by all '0s' or vice versa, or non-deterministic, featuring randomly interleaved '1s' and '0s' ~\cite{Gaines1969, B.D:journal'2001, Qian:journal'2010, Qian:journal'2011, Alaghi:ACM'2013}. The architectural simplicity of SC enables the execution of complex functions such as multiplication using merely an AND gate and a scaled addition through a simple multiplexer ~\cite{Hassan:TVLSI'2018,Hassan:TVLSI'2019}.

In digital stochastic computing (SC), the conversion from binary code to stochastic bit-streams typically relies on a component known as a stochastic number generator (SNG), which is constructed from either a random number generator (RNG) or a counter for unary scenarios, in conjunction with a comparator ~\cite{Hassan:TVLSI'2018}. The effectiveness of this conversion is predominantly measured by the ratio of '1s' to the total number of bits in the stream.
 
Within this computational model, two encoding strategies are predominant: unipolar and bipolar formats. These methods are theoretically akin and can be integrated within the same framework. The unipolar approach encodes a real number \( m \) within the interval \( 0 \leq m \leq 1 \) corresponding to a stochastic bit-stream \( M(t) \) of length \( L \), where \( t = 1, 2, \ldots, L \). In this format, the probability of each bit being '1' is given by \( P(M = 1) = m \). For instance, a value of \( x = 0.4 \) could be represented by a random stream of bits such as \( 0 \, 100 \, 011 \, 100 \), indicating that \( 40\% \) of the bits are '1s' and the remainder are zero. Conversely, the bipolar format expands the numerical range to \( -1 \leq m \leq 1 \). with the probability of a '1' in each bit determined by \( P(M = 1) = \frac{m + 1}{2} \), enabling the direct representation of negative numbers. Notably, the unipolar format offers a precision twice that of the bipolar format for the same length \( L \) of the bit-stream, the precision of the unipolar format is twice that of the bipolar format. Henceforth, unless specified otherwise, the illustrations will predominantly utilize the unipolar format.
The primary synthesis strategy in stochastic logic involves reframing logical computations into arithmetic operations predicated on probability values. Basic operations such as multiplication and scaled addition are effectively demonstrated using stochastic logic, as illustrated in Figure ~\ref{fig:sc_mult_and_add_figures}.
\begin{figure}[htbp]
\centering
\begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/sc_mulitplication_and_gate.eps}
    \caption{}
    \label{fig:ram_overall_layout}
\end{subfigure}
\begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/sc_scaled_addition_mux.eps}
    \caption{}
    \label{fig:ram_layout_zoom_in}
\end{subfigure}
\caption{Stochastic Implementation of arithmetic operations: (a) Multiplication (b) Scaled addition.}
\label{fig:sc_mult_and_add_figures}
\end{figure}
 
For instance:

\begin{numberlist}

\item Multiplication: Consider a two-input AND gate, shown in Fig. 1(a). Suppose that its inputs are two independent bit-streams \(M_1\) and \(M_2\). Its output is a bit-stream \(Y\), where
\[
\begin{aligned}
y &= P(Y = 1) = P(M_1 = 1 \text{ and } M_2 = 1) \\
&= P(M_1 = 1)P(M_2 = 1) =m_1m_2.
\end{aligned}
\]
Thus, the AND gate computes the product of the two input probability values.
\item Scaled addition: Consider the functionality of a two-input multiplexer, as represented in Fig. 1(b). This device receives two separate stochastic bit-streams, \(M_1\) and \(M_2\), and a selection bit-stream \(S\) which determines the output stream \(Y\). The outcome bit-stream \(Y\) is quantified by the probability equation given by:
\[
\begin{aligned}
y &= P(Y = 1) = P(S = 1)P(M_1 = 1) \\
&+ P(S = 0)P(M_2 = 1) \\
&= s m_1 + (1 - s) m_2.
\end{aligned}
\]
This relationship elucidates that the multiplexer aggregates the probabilities of inputs \(X_1\) and \(X_2\), adjusted by the state of the selector \(S\), thereby executing a scaled addition of the input probabilities. This process effectively integrates the selection logic with probabilistic computation, providing a dynamic method to control the flow of stochastic signals based on the condition of \(S\).
\end{numberlist}

In the evolution of stochastic computing (SC), traditional implementations have grappled with significant challenges such as high latency and extensive area requirements due to inefficiencies in generating random bit streams. To address these challenges, recent advancements have introduced a paradigm shift through the development of counting-based stochastic computing (CBSC) multipliers as described in Figure~\ref{fig:cbsc_mul_concept}. As we can clearly notice that in Figure~\ref{fig:cbsc_mul_concept} (a) describes the traditional stochastic multiplication using AND gate in which the final output is governed with a counter which counts the number of '1s' relative to length of bit streams. On the other side Figure~\ref{fig:cbsc_mul_concept} (b) described the highly efficient in terms of both computational cycles and hardware costs approach  for performing the same multiplication operation with by employing down counter. Now since we know that all the zeros in the stochastic number (SN) bitstream for w and the corresponding bits for x will have zero contribution to the final outcome, we can skip those bits altogether.This observation leads to the alternative method illustrated in Figure~\ref{fig:cbsc_mul_concept} (b) , which connects an SNG directly to the bit-counter that is activated for \( w \cdot 2^N \) cycles only.


